PXGen: A Post-hoc Explainable Method for Generative Models

With the rapid growth of generative AI in numerous applications, explainable AI (XAI) plays a crucial role in ensuring the responsible development and deployment of generative AI technologies. XAI has undergone notable advancements and widespread adoption in recent years, reflecting a concerted push to enhance the transparency, interpretability, and credibility of AI systems. Recent research emphasizes that a proficient XAI method should adhere to a set of criteria, primarily focusing on two key areas. Firstly, it should ensure the quality and fluidity of explanations, encompassing aspects like faithfulness, plausibility, completeness, and tailoring to individual needs. Secondly, the design principle of the XAI system or mechanism should cover the following factors such as reliability, resilience, the verifiability of its outputs, and the transparency of its algorithm. However, research in XAI for generative models remains relatively scarce, with little exploration into how such methods can effectively meet these criteria in that domain. In this work, we propose PXGen, a post-hoc explainable method for generative models. Given a model that needs to be explained, PXGen prepares two materials for the explanation, the Anchor set and intrinsic & extrinsic criteria. Those materials are customizable by users according to their purpose and requirements. Via the calculation of each criterion, each anchor has a set of feature values and PXGen provides examplebased explanation methods according to the feature values among all the anchors and illustrated and visualized to the users via tractable algorithms such as k-dispersion or k-center.

==> section/application.tex <==
\begin{figure*}[t]
\centering
\includegraphics[width=0.9\textwidth]{application_img/validation_app.pdf} % Reduce the figure size so that it is slightly narrower than the column.
\caption{Left: Comparing the similarity results generated by comparing the model trained with class ``0'' to the experimental model. Right: Another experiment trained the model with class ``5''. Both figures show similar trends in different removal processes. }
\label{evaluate_label0_and_5}
\end{figure*}
%small \includegraphics[width=0.9\columnwidth]
%lager \includegraphics[width=0.8\textwidth]

\begin{figure}[t]
\centering
\includegraphics[width=0.6\columnwidth]{application_img/comparsion_VAETrscIN.pdf}
\caption{We need to compare our framework with the VAE-TracIn method. For our framework, we similarly identify the most  representative and least  representative anchors, then iteratively decrease data to train the models. For the VAE-TracIn method, we need to identify the most helpful or harmful anchors and iteratively decrease data to train the models. Finally, we compare the generated similarity with the original model. } 
\label{Compare_VAE_TracIn}
\end{figure}

\label{Evaluation}
In this Section, we evaluate PXGen by giving specific purpose on the explanation and compared our work with other baselines. 

\subsection{Finding Representative Training Samples}
\label{subsec:Finding Representative Training Samples}
Determining which data is most representative for the model can be a challenging issue. The criteria for ``selecting highly representative data'' are quite vague. For example, when dealing with a dataset of dog images, the ``high representativeness'' could be based on whether the images clearly show four legs, or if they should highlight standout features like big ears, among other criteria. Here, we give a specific purpose for the XAI mission. We want to find a subset of training samples that influences  the trained model the most, or vice versa. That is, the most representative training samples. 

The test model $M$ has the similar setting in Section~\ref{4_Prepare Phase}, which is trained on a training dataset containing 5,923 images with the label ``0''. The criteria for PXGen are  conducted using MSE and KLD and the anchor set is the training dataset only.

Upon utilizing PXGen, the training dataset can be divided into four groups, and each data point is assigned an anchor value coming from the addition of the KLD and MSE values.
According to the discussion in Section~\ref{subsec: VAE_4_ClassifyPhase}, we believe that the training data within the HIHE group are the most representative, while the other groups (LILE, LIHE, HILE) are the opposite. The anchor value indicates the level of representativeness within the group, with lower values being more representative and higher values being less so.

\begin{enumerate}
\item \textit{Validation}
\label{item:Validation}

To verify whether the ``highly representative data'' identified by PXGen is indeed representative for the model, we conducted data reduction experiments. That is, remove some of the training samples and observe  the difference of the model performance after the removal. Since there is no standard criteria to measure the performance of models, we compare the image similarity between the original model $M$ and the ones with removal $M'$. Intuitively, if a model trained with the removal of non-representative samples, the generated results would be closer to the original model, compared with the ones that removes samples randomly. 

We considered three scenarios. Firstly, we trained a model $M$-HIHE using only the data from the HIHE group, meaning we removed the data from the other groups (LILE, LIHE, HILE). Secondly, we trained a model $M$-Others using training data, but removed the training data from the HIHE group in an amount equivalent to that of the other groups (LILE, LIHE, HILE), prioritizing the removal of low anchor values. Thirdly, we trained a model $M$-Random by using training data from which an amount equivalent to that of the other groups (LILE, LIHE, HILE) has been randomly removed, as a baseline. Subsequently, we compared the image similarity between the images generated by these three models (each model generated 3500 images) and the images generated by the original model $M$ (3500 images). Here, we used the Frechet Inception Distance (FID) \cite{heusel2017gans} to measure image similarity.

In Figure \ref{evaluate_label0_and_5}, we can observe the change in FID values of the three models ($M$-HIHE, $M$-Others, $M$-Random) compared to the original model $M$ as the training data is gradually reduced. It is worth noting that the FID value between $M$-HIHE (which retains only the HIHE data) and model $M$ has decreased, indicating that the data of HIHE  is representative for model $M$.

%Our goal is to verify whether the similarity of the images generated by the model would be closer to those produced by the original model when we remove data points with low representativeness from the training dataset, and conversely, whether removing data points with high representativeness  yield the opposite result. This is to validate the significance of identifying data with representativeness.

%First, we have two original models, one is trained with 5,923 images labeled as 0, and the other with 5,421 images labeled as 5 ', both come from the MNIST dataset. Then we apply PXGen to their training sets, where each data point is assigned an anchor value and categorized into one of four quadrants (Quadrant 1, 2, 3, 4).The calculation of the anchor value is the sum of KLD (Kullback-Leibler Divergence) and MSE (Mean Squared Error). We believe that data with high representativeness should have a low anchor value while being assigned to the third quadrant. Conversely, data points with high anchor values that are not assigned to the third quadrant are considered to have low representativeness.

%Subsequently, we removed data points with low representativeness from the training dataset, while we removed an equal number of high representative data points. These two modified training datasets were used to train two distinct sets of models, and we compared the similarity between images generated by models trained with the reduced training dataset and those produced by the original models using Frechet Inception Distance (FID) \cite{heusel2017gans}.Additionally, randomly removed training data was used as a baseline for comparison.

%In Figure \ref{evaluate_label0_and_5}, we observed that when we reduce the low representative data points in the training data, the images generated by the model more closely resemble those generated by the original model. However, when we reduce the high representative data points in the training data, the difference between them becomes more pronounced. This suggests that we have successfully identified a set of data points that represent the behavior of the model.

\item \textit{Comparison with TracIn:}

In this part, we compare PXGen with the VAE-TracIn~\cite{kong2021understanding} method, which evaluates an influence score to determine which training data point is most responsible for increasing the likelihood of a specific data point.  We apply VAE-TracIn to the images generated by model $M$ (3,500 images).  Therefore, for the images generated by Model $M$, each data point in the training dataset of Model $M$ has been assigned 3,500 influence scores. After averaging these scores, we obtain the influence score of this data point for the model, which represents the influence of the data point on the model's generation. In this way, all the training data have an influence score. If the training data has a high influence score, this data point is considered to be helpful for model generation, meaning it is representative. Conversely, if the training data has a low influence score, the opposite is considered true.

Referring to our setup from the previous section, we have four models ($M$, $M$-HIHE, $M$-Others, $M$-Random). In addition, we need to add a model $M$-TracIn is trained by removing the same amount of low-help (harmful) training data. Subsequently, we use $M$-HIHE, $M$-Others, $M$-Random, $M$-TracIn to compare the similarity of generated images (FID) with $M$.


In Figure~\ref{Compare_VAE_TracIn}, we individually compared the values of $M$-HIHE and $M$-TracIn, as they are both trained by removing data with low representativeness. Among them, the images generated by $M$-HIHE are more similar to those produced by the original model $M$, indicating that the training data determined by PXGen is more representative.  %The performance of PXGen and VAE-TracIn is very similar, but our advantage is that it requires less time.}

%We utilize VAE-TracIn to assess the helpful score of data points in the training data for a group of samples generated by original model. Then, each data points is assigned a score corresponding to one sample in the group. We calculate the average of all scores assigned to each data point against the group of samples, which represents its usefulness for the model.

%For PXGen, we repeat the validation experiment. For VAE-TracIn, we reduce an equal number of high  and low helpful data points and train models. and we have four set of model (high representative-PXGen,low representative-PXGen,high helpfulness,low helpfulness-PXGen) and compare their similarity using FID score with original model,which is trained with 5,923 images labeled as 0 from Mnist dataset .

%In Figure \ref{Compare_VAE_TracIn},when comparing the results of PXGen and VAE-TracIn, we found that in the comparison of FID scores between the low representative and low helpful models, result of PXGen yielded lower FID scores, indicating a closer similarity to the original model in generating samples.
\end{enumerate}





%you with certainty if the model has used specific data, but it can indirectly suggest the probability of such data being used. PXGen can divide data into four groups (LILE, LIHE, HIHE, HILE). Utilizing this feature, users can categorize the training data and calculate the proportion each group holds. This proportion implies the likelihood of specific data being used, as we use training data to predict the overall distribution. For instance, in Table XX, the probability for HIHE is XX\%, suggesting that data points allocated to HIHE have an XX\% chance of being used, while for LILE it is XX\%, meaning data points in this group only have an XX\% likelihood of having been used.

%Identify Training Samples. We train the model with a specific set of data. Another purpose is to determine whether the model has ever been trained with the given data or not. Suppose the model is trained with a certain dataset, we then collect other data that differs from the training dataset. The data that the model does not recognize is assigned a value. By calculating this value, we may distinguish whether the data sample is from the training dataset or not.

% Table 


==> section/demon-Soft-IntroVAE.tex <==

\begin{figure}[t]
\centering
\includegraphics[width=0.5\columnwidth]{Soft-IntroVAE_img/HILE_scatter.pdf}
%\caption{HIHE}
%\label{HIHE_plot_CIFAR10}
%\end{figure}

%\begin{figure}[t]
\centering
\includegraphics[width=0.6\columnwidth]{Soft-IntroVAE_img/HILE_rec.pdf}
\caption{In HILE, we discover the phenomenon of 'model delusion', where those anchors are incorrectly decoded and the model attempts to reconstruct the image with its own concept, generating automobile.}
\label{HILE_plot_CIFAR10}
\end{figure}


\begin{figure}[t]
\centering
\includegraphics[width=0.5\columnwidth]{Soft-IntroVAE_img/LIHE_scatter.pdf}
%\caption{HIHE}
%\label{HIHE_plot_CIFAR10}
%\end{figure}

%\begin{figure}[t]
\centering
\includegraphics[width=0.6\columnwidth]{Soft-IntroVAE_img/LIHE_rec.pdf}
\caption{In LIHE, we discover ``aligned conception'' in CIFAR10 automobiles, indicating that they preserve a similar concept.}
\label{LIHE_plot_CIFAR10}
\end{figure}

In Section ~\ref{sec: DemonstrationVAE}, we have introduced and demonstrated our PXGen framework using the traditional VAE model and the MNIST handwritten dataset. In this section, we would show our framework again to identify groups of Anchors with different characteristics. Compared to Section~\ref{sec: DemonstrationVAE}, Soft-IntroVAE~\cite{daniel2021soft} serves as the input model in PXGen instead of the traditional VAE model. Additionally, we employ the CIFAR10 dataset~\cite{krizhevsky2009learning} instead of the MNIST handwritten dataset to examine how our PXGen framework remains applicable even as the data becomes more complex, by selecting suitable criteria. In section ~\ref{5_Prepare Phase}, we describe our model construction, selection of the Anchor set, and the design of intrinsic and extrinsic criteria in different scenarios.

\subsection{The Model, Anchor Set, and criteria}
\label{5_Prepare Phase}

Model $M'$ is a Soft-IntroVAE model trained on the CIFAR10 dataset, in which we use 5,000 images with the ``Automobile'' category as the training set. Then, we pick 300 images from each category of the testing dataset as the anchor set. In the multi-criteria part, we choose Kullback-Leibler Divergence (KLD) as the intrinsic criterion which is the same as the Section~\ref{sec: DemonstrationVAE}. However, due to the complexity of the CIFAR10 dataset, we choose Fréchet Inception Distance (FID)~\cite{heusel2017gans} as the extrinsic criterion, since it may provide a better measurement of the difference between two complex pictures. To calculate the FID value of each sample, given the Anchor value $a$, we then take $a$ as the input of $M’$ to reconstruct the Anchor $a’$. Similar to Section 4, if the result of FID represents a relatively low value, we may infer that model $M’$ ``knows'' how to generate pictures that are similar to $a$. Through this process, we can quantify how much the model “knows” the Anchor $a$.

\subsection{Analysis Phase: Classifying Anchors and Analysis}
\label{5_ClassifyPhase}

To obtain information about Model $M’$ and acquire the distribution of the extrinsic and intrinsic criteria, we make model $M’$ generate 300 sample images. Unlike Section 4, since the CIFAR10 dataset is more complex and capturing information may be challenging, we calculate the 95th percentile instead of the maximum values as the criterion thresholds. With the aforementioned thresholds, an anchor $a$ is said to have high intrinsic affinity if and only if the KLD value of $a$ is below the average of the 95th percentile value. Otherwise, it is said to have low intrinsic affinity. Correspondingly, an anchor $a$ is said to have high extrinsic affinity if and only if the FID value of $a$ is below the threshold, and low extrinsic affinity otherwise. Additionally, we can classify the Anchor set into four different groups using the PXGen framework: HIHE, HILE, LIHE, LILE, which is similar to Section 4.

\paragraph{Analysis:} As previously introduced, HILE is referred to as 'model delusion', and LIHE is referred to as 'aligned conception'. We found similar trends in $M'$ too. Similar to the Section~\ref{sec: DemonstrationVAE}, in Figure~\ref{HILE_plot_CIFAR10}, we choose the lowest 5 percent of the intrinsic criterion (Kullback-Leibler Divergence) values as the threshold in the analysis phase. The anchor points we discovered indicate the ``concepts'' that the model has learned, which remain high intrinsic affinity. The difference from Section~\ref{sec: DemonstrationVAE} is that we choose FID as the extrinsic criterion. It shows similar trends in Section~\ref{subsec: VAE_4_ClassifyPhase}. One can see that with the FID getting higher, it includes more anchors which are not automobile at all, such as frog, airplanes, dogs, and so on. On the reconstruction part, the model still tries to generate the samples closing to automobile.

With a similar process in Section~\ref{subsec: VAE_4_ClassifyPhase}, we visualized the aligned conception in Figure~\ref{LIHE_plot_CIFAR10}. As the KLD increases gradually, it means that the model is less familiar with the concept from these anchor points. The top three images in Figure~\ref{LIHE_plot_CIFAR10} show that the concept of an automobile is clearer than those three images from the bottom. Though with the decrease in intrinsic affinity, the model is capable of reconstructing and outputting the concept that it has learned. One interesting finding is that most anchors are still automobiles but from different angles. This indicates that the model is not comfortable with pictures from different angles but can still decode them into automobiles well.




\begin{figure}[t]
\centering
\includegraphics[width=0.9\columnwidth]{visualization/PXGen_HIHE_cifar10.pdf}
\caption{Utilizing two algorithms to identify representative anchors within HIHE.}
\label{visualization_all_algorithm_cifar10}
\end{figure}

\begin{figure}[t]
\centering
\includegraphics[width=0.9\columnwidth]{visualization/PXGen_LILE_cifar10.pdf}
\caption{Utilizing two algorithms to identify representative anchors within LILE.}
\label{visualization_all_algorithm_quadran1_cifar10}
\end{figure}

\subsection{Discover Phase: Visualizing the most Characteristic Anchors}

Applying a methodology similar to that described in Section ~\ref{4_DiscoverPhase}, this Section utilizes the k-dispersion and k-center algorithms for the visualization and identification of characteristic anchors within specific groups. Upon selecting two distinct groups of anchors, designated as HIHE and LILE, the algorithmic results are illustrated in Figures ~\ref{visualization_all_algorithm_cifar10} and ~\ref{visualization_all_algorithm_quadran1_cifar10}, employing a k parameter value of 10.

The purpose of employing the k-dispersion algorithm is to discover $k$ anchors with maximal dissimilarity among themselves. In contrast, the $k$-center algorithm  identify $k$ cluster centers, each of which exhibits minimal dissimilarity compared to other anchors within the same cluster. In Figures ~\ref{visualization_all_algorithm_cifar10} and ~\ref{visualization_all_algorithm_quadran1_cifar10}, anchors identified based on  different core concepts are demonstrated. For instance, Figure ~\ref{visualization_all_algorithm_cifar10} presents results with discernible variations based on different concepts. In contrast, Figure ~\ref{visualization_all_algorithm_quadran1_cifar10} depicts a scenario in which a smaller dataset size results in the displayed anchors exhibiting increased similarity. These illustrative examples enhance an intuitive understanding of the  characteristics to each anchor group, thereby enriching the comprehension of the model.
